LeBenchmark 2.0: a Standardized, Replicable and Enhanced Framework for Self-supervised Representations of French Speech

Self-supervised learning (SSL) is at the origin of unprecedented improvements in many different domains including computer vision and natural language processing. Speech processing drastically benefitted from SSL as most of the current domain-related tasks are now being approached with pre-trained models. This work introduces LeBenchmark 2.0 an open-source framework for assessing and building SSL-equipped French speech technologies. It includes documented, large-scale and heterogeneous corpora with up to 14,000 hours of heterogeneous speech, ten pre-trained SSL wav2vec 2.0 models containing from 26 million to one billion learnable parameters shared with the community, and an evaluation protocol made of six downstream tasks to complement existing benchmarks. LeBenchmark 2.0 also presents unique perspectives on pre-trained SSL models for speech with the investigation of frozen versus fine-tuned downstream models, task-agnostic versus task-specific pre-trained models as well as a discussion on the carbon footprint of large-scale model training. Overall, the newly introduced models trained on 14,000 hours of French speech outperform multilingual and previous LeBenchmark SSL models across the benchmark but also required up to four times more energy for pre-training.

==> elsarticle-num-names.bst. <==
%%
%% This is file `elsarticle-num-names.bst'  (Version 2.1),
%% 
%% Copyright 2009-2020 Elsevier Ltd
%% 
%% This file is part of the 'Elsarticle Bundle'.
%% ---------------------------------------------
%% 
%% It may be distributed under the conditions of the LaTeX Project Public
%% License, either version 1.2 of this license or (at your option) any
%% later version.  The latest version of this license is in
%%    http://www.latex-project.org/lppl.txt
%% and version 1.2 or later is part of all distributions of LaTeX
%% version 1999/12/01 or later.
%%
%% $Id: elsarticle-num-names.bst 194 2020-11-23 11:29:27Z rishi $
%%
%% $URL: https://lenova.river-valley.com/svn/elsarticle/trunk/elsarticle-num-names.bst $
%%
%%

ENTRY
  { address
    author
    booktitle
    chapter
    collaboration
    edition
    editor
    howpublished
    institution
    journal
    key
    month
    note
    number
    organization
    pages
    publisher
    school
    series
    title
    type
    volume
    year
    url
    doi
    eprint
    pubmed
  }
  {}
  { label extra.label sort.label short.list }

INTEGERS { output.state before.all mid.sentence after.sentence after.block }

STRINGS { urlprefix doiprefix eprintprefix pubmedprefix }

FUNCTION {init.web.variables}
{
 "\URLprefix "     'urlprefix :=
 "\DOIprefix"      'doiprefix :=
 "\ArXivprefix  "   'eprintprefix :=
 "\Pubmedprefix "  'pubmedprefix :=
}

FUNCTION {init.state.consts}
{ #0 'before.all :=
  #1 'mid.sentence :=
  #2 'after.sentence :=
  #3 'after.block :=
}
STRINGS { s t}
FUNCTION {output.nonnull}
{ 's :=
  output.state mid.sentence =
    { ", " * write$ }
    { output.state after.block =
%        { add.period$ write$
        { ", " * write$
          newline$
          "\newblock " write$
        }
        { output.state before.all =
            'write$
            { add.period$ " " * write$ }
          if$
        }
      if$
      mid.sentence 'output.state :=
    }
  if$
  s
}
FUNCTION {output}
{ duplicate$ empty$
    'pop$
    'output.nonnull
  if$
}
FUNCTION {output.check}
{ 't :=
  duplicate$ empty$
    { pop$ "empty " t * " in " * cite$ * warning$ }
    'output.nonnull
  if$
}
FUNCTION {fin.entry}
{ add.period$
  write$
  newline$
}

FUNCTION {new.block}
{ output.state before.all =
    'skip$
    { after.block 'output.state := }
  if$
}
FUNCTION {new.sentence}
{ output.state after.block =
    'skip$
    { output.state before.all =
        'skip$
        { after.sentence 'output.state := }
      if$
    }
  if$
}
FUNCTION {add.blank}
{  " " * before.all 'output.state :=
}

FUNCTION {date.block}
{
  skip$
}

FUNCTION {not}
{   { #0 }
    { #1 }
  if$
}
FUNCTION {and}
{   'skip$
    { pop$ #0 }
  if$
}
FUNCTION {or}
{   { pop$ #1 }
    'skip$
  if$
}
FUNCTION {new.block.checkb}
{ empty$
  swap$ empty$
  and
    'skip$
    'new.block
  if$
}
FUNCTION {field.or.null}
{ duplicate$ empty$
    { pop$ "" }
    'skip$
  if$
}
FUNCTION {emphasize}
{ duplicate$ empty$
    { pop$ "" }
    { "\textit{" swap$ * "}" * }
  if$
}
FUNCTION {tie.or.space.prefix}
{ duplicate$ text.length$ #3 <
    { "~" }
    { " " }
  if$
  swap$
}

FUNCTION {capitalize}
{ "u" change.case$ "t" change.case$ }

FUNCTION {space.word}
{ " " swap$ * " " * }
 % Here are the language-specific definitions for explicit words.
 % Each function has a name bbl.xxx where xxx is the English word.
 % The language selected here is ENGLISH
FUNCTION {bbl.and}
{ "and"}

FUNCTION {bbl.etal}
{ "et~al." }

FUNCTION {bbl.editors}
{ "eds." }

FUNCTION {bbl.editor}
{ "ed." }

FUNCTION {bbl.edby}
{ "edited by" }

FUNCTION {bbl.edition}
{ "ed." }

FUNCTION {bbl.volume}
{ "volume" }

FUNCTION {bbl.of}
{ "of" }

FUNCTION {bbl.number}
{ "number" }

FUNCTION {bbl.nr}
{ "no." }

FUNCTION {bbl.in}
{ "in" }

FUNCTION {bbl.pages}
{ "pp." }

FUNCTION {bbl.page}
{ "p." }

FUNCTION {bbl.chapter}
{ "chapter" }

FUNCTION {bbl.techrep}
{ "Technical Report" }

FUNCTION {bbl.mthesis}
{ "Master's thesis" }

FUNCTION {bbl.phdthesis}
{ "Ph.D. thesis" }

MACRO {jan} {"January"}

MACRO {feb} {"February"}

MACRO {mar} {"March"}

MACRO {apr} {"April"}

MACRO {may} {"May"}

MACRO {jun} {"June"}

MACRO {jul} {"July"}

MACRO {aug} {"August"}

MACRO {sep} {"September"}

MACRO {oct} {"October"}

MACRO {nov} {"November"}

MACRO {dec} {"December"}

MACRO {acmcs} {"ACM Comput. Surv."}

MACRO {acta} {"Acta Inf."}

MACRO {cacm} {"Commun. ACM"}

MACRO {ibmjrd} {"IBM J. Res. Dev."}

MACRO {ibmsj} {"IBM Syst.~J."}

MACRO {ieeese} {"IEEE Trans. Software Eng."}

MACRO {ieeetc} {"IEEE Trans. Comput."}

MACRO {ieeetcad}
 {"IEEE Trans. Comput. Aid. Des."}

MACRO {ipl} {"Inf. Process. Lett."}

MACRO {jacm} {"J.~ACM"}

MACRO {jcss} {"J.~Comput. Syst. Sci."}

MACRO {scp} {"Sci. Comput. Program."}

MACRO {sicomp} {"SIAM J. Comput."}

MACRO {tocs} {"ACM Trans. Comput. Syst."}

MACRO {tods} {"ACM Trans. Database Syst."}

MACRO {tog} {"ACM Trans. Graphic."}

MACRO {toms} {"ACM Trans. Math. Software"}

MACRO {toois} {"ACM Trans. Office Inf. Syst."}

MACRO {toplas} {"ACM Trans. Progr. Lang. Syst."}

MACRO {tcs} {"Theor. Comput. Sci."}

FUNCTION {bibinfo.check}
{ swap$
  duplicate$ missing$
    {
      pop$ pop$
      ""
    }
    { duplicate$ empty$
        {
          swap$ pop$
        }
        { swap$
          "\bibinfo{" swap$ * "}{" * swap$ * "}" *
        }
      if$
    }
  if$
}
FUNCTION {bibinfo.warn}
{ swap$
  duplicate$ missing$
    {
      swap$ "missing " swap$ * " in " * cite$ * warning$ pop$
      ""
    }
    { duplicate$ empty$
        {
          swap$ "empty " swap$ * " in " * cite$ * warning$
        }
        { swap$
          pop$
        }
      if$
    }
  if$
}
STRINGS  { bibinfo}
INTEGERS { nameptr namesleft numnames }

FUNCTION {format.names}
{ 'bibinfo :=
  duplicate$ empty$ 'skip$ {
  's :=
  "" 't :=
  #1 'nameptr :=
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr
      "{f.~}{vv~}{ll}{, jj}"
      format.name$
      bibinfo bibinfo.check
      't :=
      nameptr #1 >
        {
          namesleft #1 >
            { ", " * t * }
            {
              "," *
              s nameptr "{ll}" format.name$ duplicate$ "others" =
                { 't := }
                { pop$ }
              if$
              t "others" =
                {
                  " " * bbl.etal *
                }
                { " " * t * }
              if$
            }
          if$
        }
        't
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
  } if$
}
FUNCTION {format.names.ed}
{
  format.names
}
FUNCTION {format.key}
{ empty$
    { key field.or.null }
    { "" }
  if$
}

%FUNCTION {format.authors}
%{ author "author" format.names
%}

FUNCTION {format.authors}
{ author "author" format.names
    duplicate$ empty$ 'skip$
    { collaboration "collaboration" bibinfo.check
      duplicate$ empty$ 'skip$
        { " (" swap$ * ")" * }
      if$
      *
    }
  if$
}

FUNCTION {get.bbl.editor}
{ editor num.names$ #1 > 'bbl.editors 'bbl.editor if$ }

FUNCTION {format.editors}
{ editor "editor" format.names duplicate$ empty$ 'skip$
    {
      " " *
      get.bbl.editor
      capitalize
   "(" swap$ * ")" *
      *
    }
  if$
}
FUNCTION {format.note}
{
 note empty$
    { "" }
    { note #1 #1 substring$
      duplicate$ "{" =
        'skip$
        { output.state mid.sentence =
          { "l" }
          { "u" }
        if$
        change.case$
        }
      if$
      note #2 global.max$ substring$ * "note" bibinfo.check
    }
  if$
}

FUNCTION {format.title}
{ title
  duplicate$ empty$ 'skip$
    { "t" change.case$ }
  if$
  "title" bibinfo.check
}

FUNCTION {format.full.names}
{'s :=
 "" 't :=
 #1 'nameptr :=
 s num.names$ 'numnames :=
 numnames 'namesleft :=
   { namesleft #0 > }
   { s nameptr
     "{vv~}{ll}" format.name$
     't :=
     nameptr #1 >
       {
         namesleft #1 >
           { ", " * t * }
           {
             s nameptr "{ll}" format.name$ duplicate$ "others" =
               { 't := }
               { pop$ }
             if$
             t "others" =
               {
                 " " * bbl.etal *
               }
               {
                 numnames #2 >
                   { "," * }
                   'skip$
                 if$
                 bbl.and
                 space.word * t *
               }
             if$
           }
         if$
       }
       't
     if$
     nameptr #1 + 'nameptr :=
     namesleft #1 - 'namesleft :=
   }
 while$
}

FUNCTION {author.editor.key.full}
{ author empty$
   { editor empty$
       { key empty$
           { cite$ #1 #3 substring$ }
           'key
         if$
       }
       { editor format.full.names }
     if$
   }
   { author format.full.names }
 if$
}

FUNCTION {author.key.full}
{ author empty$
   { key empty$
        { cite$ #1 #3 substring$ }
         'key
     if$
   }
   { author format.full.names }
 if$
}

FUNCTION {editor.key.full}
{ editor empty$
   { key empty$
        { cite$ #1 #3 substring$ }
         'key
     if$
   }
   { editor format.full.names }
 if$
}

FUNCTION {make.full.names}
{ type$ "book" =
 type$ "inbook" =
 or
   'author.editor.key.full
   { type$ "proceedings" =
       'editor.key.full
       'author.key.full
     if$
   }
 if$
}

FUNCTION {output.bibitem}
{ newline$
 "\bibitem[{" write$
 label write$
 ")" make.full.names duplicate$ short.list =
    { pop$ }
    { * }
  if$
 "}]{" * write$
 cite$ write$
 "}" write$
 newline$
 ""
 before.all 'output.state :=
}

FUNCTION {n.dashify}
{
  't :=
  ""
    { t empty$ not }
    { t #1 #1 substring$ "-" =
        { t #1 #2 substring$ "--" = not
            { "--" *
              t #2 global.max$ substring$ 't :=
            }
            {   { t #1 #1 substring$ "-" = }
                { "-" *
                  t #2 global.max$ substring$ 't :=
                }
              while$
            }
          if$
        }
        { t #1 #1 substring$ *
          t #2 global.max$ substring$ 't :=
        }
      if$
    }
  while$
}

FUNCTION {word.in}
{ bbl.in
  ":" *
  " " * }

FUNCTION {format.date}
{ year "year" bibinfo.check duplicate$ empty$
    {
      "empty year in " cite$ * "; set to ????" * warning$
       pop$ "????"
    }
    'skip$
  if$
  extra.label *
}
FUNCTION{format.year}
{ year "year" bibinfo.check duplicate$ empty$
    {  "empty year in " cite$ *
       "; set to ????" *
       warning$
       pop$ "????"
    }
    {
    }
  if$
  extra.label *
  " (" swap$ * ")" *
}
FUNCTION {format.btitle}
{ title "title" bibinfo.check
  duplicate$ empty$ 'skip$
    {
    }
  if$
}
FUNCTION {either.or.check}
{ empty$
    'pop$
    { "can't use both " swap$ * " fields in " * cite$ * warning$ }
  if$
}
FUNCTION {format.bvolume}
{ volume empty$
    { "" }
    { bbl.volume volume tie.or.space.prefix
      "volume" bibinfo.check * *
      series "series" bibinfo.check
      duplicate$ empty$ 'pop$
        { swap$ bbl.of space.word * swap$
          emphasize * }
      if$
      "volume and number" number either.or.check
    }
  if$
}
FUNCTION {format.number.series}
{ volume empty$
    { number empty$
        { series field.or.null }
        { series empty$
            { number "number" bibinfo.check }
        { output.state mid.sentence =
            { bbl.number }
            { bbl.number capitalize }
          if$
          number tie.or.space.prefix "number" bibinfo.check * *
          bbl.in space.word *
          series "series" bibinfo.check *
        }
      if$
    }
      if$
    }
    { "" }
  if$
}

FUNCTION {format.edition}
{ edition duplicate$ empty$ 'skip$
    {
      output.state mid.sentence =
        { "l" }
        { "t" }
      if$ change.case$
      "edition" bibinfo.check
      " " * bbl.edition *
    }
  if$
}
INTEGERS { multiresult }
FUNCTION {multi.page.check}
{ 't :=
  #0 'multiresult :=
    { multiresult not
      t empty$ not
      and
    }
    { t #1 #1 substring$
      duplicate$ "-" =
      swap$ duplicate$ "," =
      swap$ "+" =
      or or
        { #1 'multiresult := }
        { t #2 global.max$ substring$ 't := }
      if$
    }
  while$
  multiresult
}
FUNCTION {format.pages}
{ pages duplicate$ empty$ 'skip$
    { duplicate$ multi.page.check
        {
          bbl.pages swap$
          n.dashify
        }
        {
          bbl.page swap$
        }
      if$
      tie.or.space.prefix
      "pages" bibinfo.check
      * *
    }
  if$
}
FUNCTION {format.journal.pages}
{ pages duplicate$ empty$ 'pop$
    { swap$ duplicate$ empty$
        { pop$ pop$ format.pages }
        {
          " " *
          swap$
          n.dashify
          "pages" bibinfo.check
          *
        }
      if$
    }
  if$
}
FUNCTION {format.vol.num.pages}
{ volume field.or.null
  duplicate$ empty$ 'skip$
    {
      "volume" bibinfo.check
    }
  if$
  format.year *
}

FUNCTION {format.chapter.pages}
{ chapter empty$
    { "" }
    { type empty$
        { bbl.chapter }
        { type "l" change.case$
          "type" bibinfo.check
        }
      if$
      chapter tie.or.space.prefix
      "chapter" bibinfo.check
      * *
    }
  if$
}

FUNCTION {format.booktitle}
{
  booktitle "booktitle" bibinfo.check
}
FUNCTION {format.in.ed.booktitle}
{ format.booktitle duplicate$ empty$ 'skip$
    {
      editor "editor" format.names.ed duplicate$ empty$ 'pop$
        {
          " " *
          get.bbl.editor
          capitalize
          "(" swap$ * "), " *
          * swap$
          * }
      if$
      word.in swap$ *
    }
  if$
}
FUNCTION {format.thesis.type}
{ type duplicate$ empty$
    'pop$
    { swap$ pop$
      "t" change.case$ "type" bibinfo.check
    }
  if$
}
FUNCTION {format.tr.number}
{ number "number" bibinfo.check
  type duplicate$ empty$
    { pop$ bbl.techrep }
    'skip$
  if$
  "type" bibinfo.check
  swap$ duplicate$ empty$
    { pop$ "t" change.case$ }
    { tie.or.space.prefix * * }
  if$
}
FUNCTION {format.article.crossref}
{
  word.in
  " \cite{" * crossref * "}" *
}
FUNCTION {format.book.crossref}
{ volume duplicate$ empty$
    { "empty volume in " cite$ * "'s crossref of " * crossref * warning$
      pop$ word.in
    }
    { bbl.volume
      swap$ tie.or.space.prefix "volume" bibinfo.check * * bbl.of space.word *
    }
  if$
  " \cite{" * crossref * "}" *
}
FUNCTION {format.incoll.inproc.crossref}
{
  word.in
  " \cite{" * crossref * "}" *
}
FUNCTION {format.org.or.pub}
{ 't :=
  ""
  address empty$ t empty$ and
    'skip$
    {
      t empty$
        { address "address" bibinfo.check *
        }
        { t *
          address empty$
            'skip$
            { ", " * address "address" bibinfo.check * }
          if$
        }
      if$
    }
  if$
}
FUNCTION {format.publisher.address}
{ publisher "publisher" bibinfo.check format.org.or.pub
}

FUNCTION {format.organization.address}
{ organization "organization" bibinfo.check format.org.or.pub
}

FUNCTION {print.url}
 {url duplicate$ empty$
   { pop$ "" }
   { new.sentence
     urlprefix "\url{" * swap$  * "}" *
   }
   if$
 }

FUNCTION {print.doi}
 {doi duplicate$ empty$
   { pop$ "" }
   { new.sentence
     doiprefix "\doi{" * swap$  * "}" *
   }
   if$
 }

FUNCTION {print.eprint}
 {eprint duplicate$ empty$
   { pop$ "" }
   { new.sentence
     duplicate$ "\href{http://arxiv.org/abs/" swap$ * "}{{\tt arXiv:" * swap$ * "}}" *
   }
   if$
 }

FUNCTION {print.pubmed}
 {pubmed duplicate$ empty$
   { pop$ "" }
   { new.sentence
     pubmedprefix "\Pubmed{" * swap$  * "}" *
   }
   if$
 }

FUNCTION {webpage}
{ "%Type = Webpage" write$
  output.bibitem
  format.authors "author" output.check
  author format.key output
  author empty$
  {
    format.title "title" output.check
    new.block
    format.date "year" output.check
    date.block
  }
  {
    format.date "year" output.check
    date.block
    format.title "title" output.check
    new.block
}
  if$
  print.url output
  fin.entry
}


FUNCTION {article}
{ "%Type = Article" write$
  output.bibitem
  format.authors "author" output.check
  author format.key output
  new.block
  format.title "title" output.check
  new.block
  crossref missing$
    {
      journal
      "journal" bibinfo.check
      "journal" output.check
      add.blank
      format.vol.num.pages output
    }
    { format.article.crossref output.nonnull
    }
  if$
  format.journal.pages
  new.sentence
  print.url output
  print.doi output
  print.eprint output
  print.pubmed output
  format.note output
  fin.entry
}
FUNCTION {book}
{ "%Type = Book" write$
  output.bibitem
  author empty$
    { format.editors "author and editor" output.check
      editor format.key output
    }
    { format.authors output.nonnull
      crossref missing$
        { "author and editor" editor either.or.check }
        'skip$
      if$
    }
  if$
  format.btitle "title" output.check
  crossref missing$
    { format.bvolume output
      format.number.series output
      format.edition output
      format.publisher.address output
    }
    {
      format.book.crossref output.nonnull
    }
  if$
  format.date "year" output.check
  new.sentence
  print.url output
  print.doi output
  print.eprint output
  print.pubmed output
  format.note output
  fin.entry
}
FUNCTION {booklet}
{ "%Type = Booklet" write$
  output.bibitem
  format.authors output
  author format.key output
  format.title "title" output.check
  howpublished "howpublished" bibinfo.check output
  address "address" bibinfo.check output
  format.date "year" output.check
  new.sentence
  print.url output
  print.doi output
  print.eprint output
  print.pubmed output
  format.note output
  fin.entry
}

FUNCTION {inbook}
{ "%Type = Inbook" write$
  output.bibitem
  author empty$
    { format.editors "author and editor" output.check
      editor format.key output
    }
    { format.authors output.nonnull
      crossref missing$
        { "author and editor" editor either.or.check }
        'skip$
      if$
    }
  if$
  format.btitle "title" output.check
  crossref missing$
    {
      format.bvolume output
      format.number.series output
      format.edition output
      format.publisher.address output
    }
    {
      format.book.crossref output.nonnull
    }
  if$
  format.date "year" output.check
  format.pages "pages" output.check
  new.sentence
  print.url output
  print.doi output
  print.eprint output
  print.pubmed output
  format.note output
  fin.entry
}

FUNCTION {incollection}
{ "%Type = Incollection" write$
  output.bibitem
  format.authors "author" output.check
  author format.key output
  new.block
  format.title "title" output.check
  new.block
  crossref missing$
    { format.in.ed.booktitle "booktitle" output.check
      format.bvolume output
      format.number.series output
      format.edition output
      format.publisher.address output
    }
    { format.incoll.inproc.crossref output.nonnull
    }
  if$
  format.date "year" output.check
  format.pages "pages" output.check
  new.sentence
  print.url output
  print.doi output
  print.eprint output
  print.pubmed output
  format.note output
  fin.entry
}
FUNCTION {inproceedings}
{ "%Type = Inproceedings" write$
  output.bibitem
  format.authors "author" output.check
  author format.key output
  new.block
  format.title "title" output.check
  new.block
  crossref missing$
    { format.in.ed.booktitle "booktitle" output.check
      format.bvolume output
      format.number.series output
      publisher empty$
        { format.organization.address output }
        { organization "organization" bibinfo.check output
          format.publisher.address output
        }
      if$
    }
    { format.incoll.inproc.crossref output.nonnull
    }
  if$
  format.date output
  format.pages "pages" output.check
  new.sentence
  print.url output
  print.doi output
  print.eprint output
  print.pubmed output
  format.note output
  fin.entry
}
FUNCTION {conference} { inproceedings }
FUNCTION {manual}
{ "%Type = Manual" write$
  output.bibitem
  format.authors output
  author format.key output
  format.btitle "title" output.check
  format.edition output
  organization "organization" bibinfo.check output
  address "address" bibinfo.check output
  format.date "year" output.check
  new.sentence
  print.url output
  print.doi output
  print.eprint output
  print.pubmed output
  format.note output
  fin.entry
}

FUNCTION {mastersthesis}
{ "%Type = Masterthesis" write$
  output.bibitem
  format.authors "author" output.check
  author format.key output
  format.btitle
  "title" output.check
  bbl.mthesis format.thesis.type output.nonnull
  school "school" bibinfo.warn output
  address "address" bibinfo.check output
  format.date "year" output.check
  new.sentence
  print.url output
  print.doi output
  print.eprint output
  print.pubmed output
  format.note output
  fin.entry
}

FUNCTION {misc}
{ "%Type = Misc" write$
  output.bibitem
  format.authors output
  author format.key output
  format.title output
  howpublished "howpublished" bibinfo.check output
  format.date "year" output.check
  new.sentence
  print.url output
  print.doi output
  print.eprint output
  print.pubmed output
  format.note output
  fin.entry
}
FUNCTION {phdthesis}
{ "%Type = Phdthesis" write$
  output.bibitem
  format.authors "author" output.check
  author format.key output
  format.btitle
  "title" output.check
  bbl.phdthesis format.thesis.type output.nonnull
  school "school" bibinfo.warn output
  address "address" bibinfo.check output
  format.date "year" output.check
  new.sentence
  print.url output
  print.doi output
  print.eprint output
  print.pubmed output
  format.note output
  fin.entry
}

FUNCTION {proceedings}
{ "%Type = Proceedings" write$
  output.bibitem
  format.editors output
  editor format.key output
  format.btitle "title" output.check
  format.bvolume output
  format.number.series output
  publisher empty$
    { format.organization.address output }
    { organization "organization" bibinfo.check output
      format.publisher.address output
    }
  if$
  format.date "year" output.check
  new.sentence
  print.url output
  print.doi output
  print.eprint output
  print.pubmed output
  format.note output
  fin.entry
}

FUNCTION {techreport}
{ "%Type = Techreport" write$
  output.bibitem
  format.authors "author" output.check
  author format.key output
  format.btitle
  "title" output.check
  format.tr.number output.nonnull
  institution "institution" bibinfo.warn output
  address "address" bibinfo.check output
  format.date "year" output.check
  new.sentence
  print.url output
  print.doi output
  print.eprint output
  print.pubmed output
  format.note output
  fin.entry
}

FUNCTION {unpublished}
{ "%Type = Unpublished" write$
  output.bibitem
  format.authors "author" output.check
  author format.key output
  format.title "title" output.check
  format.date "year" output.check
  new.sentence
  print.url output
  print.doi output
  print.eprint output
  print.pubmed output
  format.note "note" output.check
  fin.entry
}

FUNCTION {default.type} { misc }
READ
FUNCTION {sortify}
{ purify$
  "l" change.case$
}
INTEGERS { len }
FUNCTION {chop.word}
{ 's :=
  'len :=
  s #1 len substring$ =
    { s len #1 + global.max$ substring$ }
    's
  if$
}
FUNCTION {format.lab.names}
{ 's :=
  "" 't :=
  s #1 "{vv~}{ll}" format.name$
  s num.names$ duplicate$
  #2 >
    { pop$
      " " * bbl.etal *
    }
    { #2 <
        'skip$
        { s #2 "{ff }{vv }{ll}{ jj}" format.name$ "others" =
            {
              " " * bbl.etal *
            }
            { bbl.and space.word * s #2 "{vv~}{ll}" format.name$
              * }
          if$
        }
      if$
    }
  if$
}

FUNCTION {author.key.label}
{ author empty$
    { key empty$
        { cite$ #1 #3 substring$ }
        'key
      if$
    }
    { author format.lab.names }
  if$
}

FUNCTION {author.editor.key.label}
{ author empty$
    { editor empty$
        { key empty$
            { cite$ #1 #3 substring$ }
            'key
          if$
        }
        { editor format.lab.names }
      if$
    }
    { author format.lab.names }
  if$
}

FUNCTION {editor.key.label}
{ editor empty$
    { key empty$
        { cite$ #1 #3 substring$ }
        'key
      if$
    }
    { editor format.lab.names }
  if$
}

FUNCTION {calc.short.authors}
{ type$ "book" =
  type$ "inbook" =
  or
    'author.editor.key.label
    { type$ "proceedings" =
        'editor.key.label
        'author.key.label
      if$
    }
  if$
  'short.list :=
}

FUNCTION {calc.label}
{ calc.short.authors
  short.list
  "("
  *
  year duplicate$ empty$
     { pop$ "????" }
     { purify$ #-1 #4 substring$ }
  if$
  *
  'label :=
}

FUNCTION {sort.format.names}
{ 's :=
  #1 'nameptr :=
  ""
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr
      "{vv{ } }{ll{ }}{  f{ }}{  jj{ }}"
      format.name$ 't :=
      nameptr #1 >
        {
          "   "  *
          namesleft #1 = t "others" = and
            { "zzzzz" * }
            { t sortify * }
          if$
        }
        { t sortify * }
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
}

FUNCTION {sort.format.title}
{ 't :=
  "A " #2
    "An " #3
      "The " #4 t chop.word
    chop.word
  chop.word
  sortify
  #1 global.max$ substring$
}
FUNCTION {author.sort}
{ author empty$
    { key empty$
        { "to sort, need author or key in " cite$ * warning$
          ""
        }
        { key sortify }
      if$
    }
    { author sort.format.names }
  if$
}
FUNCTION {author.editor.sort}
{ author empty$
    { editor empty$
        { key empty$
            { "to sort, need author, editor, or key in " cite$ * warning$
              ""
            }
            { key sortify }
          if$
        }
        { editor sort.format.names }
      if$
    }
    { author sort.format.names }
  if$
}
FUNCTION {editor.sort}
{ editor empty$
    { key empty$
        { "to sort, need editor or key in " cite$ * warning$
          ""
        }
        { key sortify }
      if$
    }
    { editor sort.format.names }
  if$
}
FUNCTION {presort}
{ calc.label
  label sortify
  "    "
  *
  type$ "book" =
  type$ "inbook" =
  or
    'author.editor.sort
    { type$ "proceedings" =
        'editor.sort
        'author.sort
      if$
    }
  if$
  #1 entry.max$ substring$
  'sort.label :=
  sort.label
  *
  "    "
  *
  title field.or.null
  sort.format.title
  *
  #1 entry.max$ substring$
  'sort.key$ :=
}

ITERATE {presort}
%SORT
STRINGS { last.label next.extra }
INTEGERS { last.extra.num number.label }
FUNCTION {initialize.extra.label.stuff}
{ #0 int.to.chr$ 'last.label :=
  "" 'next.extra :=
  #0 'last.extra.num :=
  #0 'number.label :=
}
FUNCTION {forward.pass}
{ last.label label =
    { last.extra.num #1 + 'last.extra.num :=
      last.extra.num int.to.chr$ 'extra.label :=
    }
    { "a" chr.to.int$ 'last.extra.num :=
      "" 'extra.label :=
      label 'last.label :=
    }
  if$
  number.label #1 + 'number.label :=
}
FUNCTION {reverse.pass}
{ next.extra "b" =
    { "a" 'extra.label := }
    'skip$
  if$
  extra.label 'next.extra :=
  extra.label
  duplicate$ empty$
    'skip$
    { "{\natexlab{" swap$ * "}}" * }
  if$
  'extra.label :=
  label extra.label * 'label :=
}
EXECUTE {initialize.extra.label.stuff}
ITERATE {forward.pass}
REVERSE {reverse.pass}
FUNCTION {bib.sort.order}
{ sort.label
  "    "
  *
  year field.or.null sortify
  *
  "    "
  *
  title field.or.null
  sort.format.title
  *
  #1 entry.max$ substring$
  'sort.key$ :=
}
ITERATE {bib.sort.order}
%SORT
FUNCTION {begin.bib}
{ preamble$ empty$
    'skip$
    { preamble$ write$ newline$ }
  if$
  "\begin{thebibliography}{" number.label int.to.str$ * "}" *
  write$ newline$
  "\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi"
  write$ newline$
  "\providecommand{\url}[1]{\texttt{#1}}"
  write$ newline$
  "\providecommand{\href}[2]{#2}"
  write$ newline$
  "\providecommand{\path}[1]{#1}"
  write$ newline$
  "\providecommand{\DOIprefix}{doi:}"
  write$ newline$
  "\providecommand{\ArXivprefix}{arXiv:}"
  write$ newline$
  "\providecommand{\URLprefix}{URL: }"
  write$ newline$
  "\providecommand{\Pubmedprefix}{pmid:}"
  write$ newline$
  "\providecommand{\doi}[1]{\href{http://dx.doi.org/#1}{\path{#1}}}"
  write$ newline$
  "\providecommand{\Pubmed}[1]{\href{pmid:#1}{\path{#1}}}"
  write$ newline$
  "\providecommand{\bibinfo}[2]{#2}"
  write$ newline$
	"\ifx\xfnm\relax \def\xfnm[#1]{\unskip,\space#1}\fi"
  write$ newline$
}
EXECUTE {begin.bib}
EXECUTE {init.state.consts}
EXECUTE {init.web.variables} 
ITERATE {call.type$}
FUNCTION {end.bib}
{ newline$
  "\end{thebibliography}" write$ newline$
}
EXECUTE {end.bib}
%% End of customized bst file
%%
%% End of file `elsarticle-num-names.bst'.
%%
%%
%% Change log:
%% -----------
%% 22.04.2011
%%
%% 10.08.2012
%%   a. doi, url, eprint, pmid added
%%   b. Bibtype `webpage' defined
%%
%% 30.08.2012
%%   a. collaboration added.




==> tables/SLU_table1.tex <==
\begin{table}[!t]
\caption{End2End SLU results in concept error rate (CER \%, lower is better $\shpos$) on the MEDIA corpus. ``h256'' and ``h300'' refer to a hidden size of 256 and 300 and neurons respectively, while ``mt'' is a multi-task ASR-SLU training. ``t2'' means that a Softmax temperature of value 2 was applied.}
\scriptsize
\begin{center}
\scalebox{1}{
    \begin{tabular}{l|c|c|c|c|c}

        \toprule
        \multicolumn{6}{c}{Corpus: MEDIA, Metric: Concept Error Rate (CER \%) $\shpos$} \\
        \midrule
        \textbf{Model} & \textbf{Params (SSL/SLU)} & \textbf{Representation} & \textbf{RawER} & \textbf{Dev} & \textbf{Test} \\
        \midrule
        %\hline
        \multicolumn{6}{c}{\textbf{Task-agnostic models}} \\
        \hline
         h300 &   -/13.18 & spectrogram & 59.36 &    64.96  &   58.12 \\
         h300 mt &   -/13.18 & spectrogram & \textbf{30.44} &    30.24 &   \textbf{30.39} \\
        \midrule
        %\hline
         h256 \citep{lebenchmark2} &   330/12.18 & 7K-\textit{large} & - &    19.68  &   18.77 \\
        % h256 &   308/12.18 & w2v2 7k L & 16.50 &   17.16  &    \textbf{15.39} \\
        % h256 mt &   308/12.18 & w2v2 7k L & \textbf{15.40} &    16.86  &   \textbf{15.36} \\
         h300 &   330/15.45 & 7K-\textit{large} & 17.26 &    18.57  &   16.99 \\
         h300 mt &   330/15.45 & 7K-\textit{large} & \textbf{15.36} &    \textbf{16.62}  &   \textbf{15.47} \\
        \hline
         h256 &   26/12.18 & 14K-\textit{light} & 22.71 & 22.62 & 20.92 \\
         h256 mt &   26/12.18 & 14K-\textit{light} & \textbf{19.29} & \textbf{19.41} & \textbf{18.67} \\
        % h300 &   26/12.18 & w2v2 14k XS & 22.81 & 23.62 & 22.53 \\
        % h300 mt &   26/12.18 & w2v2 14k XS & 19.36 & 20.07 & 19.16 \\
        \hline
        % h256 &   308/12.18 & w2v2 14k L & 16.05 & 17.04 & 15.67 \\
        % h256 mt &   308/12.18 & w2v2 14k L & 16.28 & 17.79 & \textbf{14.47} \\
         h300 &   330/15.45 & 14K-\textit{large} & 18.26 & 18.63 & 17.35 \\
         h300 mt &   330/15.45 & 14K-\textit{large} & \textbf{15.91} & \textbf{16.62} & \textbf{14.43} \\
        \hline
         h256 &    965/12.70 & 14K-\textit{xlarge} & 21.44 & 17.52 & 16.24 \\
         h256 mt &    965/12.70 & 14K-\textit{xlarge} & \textbf{14.73} & \textbf{15.66} & \textbf{14.43} \\
        % h300 &    1000/16.07 & w2v2 14k XL & 18.34 &   19.29 & 16.38 \\
        % h300 mt &    1000/16.07 & w2v2 14k XL & 15.27 & \textbf{15.66} & 15.37 \\
        \midrule
        %\hline
         h256 \citep{lebenchmark2} &    330/12.18 & XLSR-53-\textit{large} & - & \textbf{18.45} & 18.78 \\
         h256 &    330/12.18 & XLSR-53-\textit{large} & 18.38 & 18.99 & 18.68 \\
         h256 mt &    330/12.18 & XLSR-53-\textit{large} & \textbf{17.74} & 18.84 & \textbf{17.16} \\
        % h300 &    308/15.45 & xlsr-53 L & 22.36 & 23.25 & 22.01 \\
        % h300 mt &    308/15.45 & xlsr-53 L & 18.11 & 19.05 & \textbf{16.66} \\
        \hline
        % h256 &    1000/12.70 & xlsr-53 XL & \textbf{14.81} & 18.77 & 30.05 \\
        % h256 mt &    1000/12.70 & xlsr-53 XL & 18.15 & 19.09 & 30.98 \\
         h300 &    965/16.07 & XLS-R-\textit{xlarge} & 18.02 & 20.75 & 30.08 \\
         h300 mt &    965/16.07 & XLS-R-\textit{xlarge} & 18.53 & \textbf{18.57} & \textbf{29.07} \\
        \hline
        %\hline
         h256 &   244/11.66 & whisper-s & 27.86 &     \textbf{28.44}  &   27.19 \\
         h256 &   769/12.18 & whisper-m & 34.03 &    33.75  &   31.10 \\
         h256 &   1550/12.71 & whisper-l & \textbf{26.39} &   28.92  &   \textbf{26.90} \\
        \midrule
        %\hline
        \multicolumn{6}{c}{\textbf{Task-specific models (ASR fine-tuning)}} \\
        \hline
         h256 \citep{lebenchmark2}           &   330/12.18 & 7K-\textit{large} & - & 14.58 & 13.78 \\
        % h256           &   308/12.18 & w2v2-fr-7k L & 13.79 & 14.07 & 12.67 \\
        % h256 mt           &   308/12.18 & w2v2-fr-7k L & \textbf{10.71} & 14.43 & \textbf{12.52} \\
         h300 t2          &   330/15.45 & 7K-\textit{large} & 10.82 & \textbf{13.53} & 12.80 \\ % n.a. without t2
         h300 mt t2           &   330/15.45 & 7K-\textit{large} & 10.83 & 13.95 & \textbf{12.71} \\
        \hline
        % h256           &   26/12.18 & w2v2-fr-14k XS & 14.62 & 17.94 & 19.36 \\
        % h256 mt          &   26/12.18 & w2v2-fr-14k XS & 16.28 & 16.32 & 19.64 \\
         h300           &   26/15.45 & 14K-\textit{light} & 15.07 & 17.03 & 20.02 \\
         h300 mt          &   26/15.45 & 14K-\textit{light} & \textbf{13.66} & \textbf{15.48} & \textbf{18.22} \\
        \hline
         h256 t2           &   330/12.18 & 14K-\textit{large} & \textbf{10.43} & \textbf{12.96} & 13.78 \\
         h256 mt t2          &   330/12.18 & 14K-\textit{large} & 13.76 & 14.43 & \textbf{12.85} \\
        % h300 t2           &   308/15.45 & w2v2-fr-14k L & 11.06 & 13.71 & 13.48 \\
        % h300 mt t2          &   308/15.45 & w2v2-fr-14k L & 11.11 & 14.28 & 13.88 \\
        \hline
         h256 t2           &   965/12.70 & 14K-\textit{xlarge} & \textbf{11.19} & \textbf{13.74} & \textbf{13.88} \\
         h256 mt t2          &   965/12.70 & 14K-\textit{xlarge} & 11.35 & 14.58 & 14.53 \\
        % h300 t2           &   1000/16.07 & w2v2-fr-14k XL & 11.64 & 14.19 & \textbf{13.77} \\
        % h300 mt t2          &   1000/16.07 & w2v2-fr-14k XL & 17.96 & 20.73 & \textbf{13.69} \\
        \midrule
        %\hline
        % h256          &   308/12.18 & xlsr53 L & 17.21 & 15.78 & \textbf{15.00} \\
        % h256 mt         &   308/12.18 & xlsr53 L & 14.66 & 15.87 & 17.70 \\
         h300          &   330/15.45 & XLSR-53-\textit{large} & 18.45 & 17.42 & \textbf{15.01} \\
         h300 mt         &   330/15.45 & XLSR-53-\textit{large} & \textbf{13.09} & \textbf{15.22} & 16.60 \\
        \hline
        % h256           &   1000/12.70 & xlsr53 XL & 13.87 & 15.60 & 24.13 \\
        % h256 mt          &   1000/12.70 & xlsr53 XL & 15.00 & 16.08 & 24.84 \\
         h300 t2          &   965/16.07 & XLS-R-\textit{xlarge} & 14.87 & 17.22 & 24.15 \\
         h300 mt t2          &   965/16.07 & XLS-R-\textit{xlarge} & \textbf{13.39} & \textbf{15.42} & \textbf{23.30} \\
        \hline
        
    \end{tabular}
}
\end{center}
\label{tab:SLU-MEDIA-results}
\end{table}

==> tables/corpora_table.tex <==

\begin{table*}[!htb]
\caption{Statistics for the speech corpora used to train SSL models according to gender information (male / female / unknown). 
The small dataset is from MLS only. Every dataset is composed of the previous one + additional data; %MPF, TCOF and CFPP2000 appear twice with different stats as data extraction changed; 
duration: hour(s):minute(s).}
%}
\centering
\scalebox{0.85}{
\scriptsize
\begin{tabular}{lccccc}\toprule

\textbf{Corpus$_{License}$}                                                    & \textbf{\# Utterances}               & \textbf{Duration}                    & \textbf{\# Speakers} & \textbf{Mean Utt. Duration} & \textbf{Speech type}\\

\midrule
%&&&&& \\
\multicolumn{6}{c}{\textbf{Small dataset -- 1K}} \\ \hline

MLS French$_{CC BY 4.0}$~\citep{old_pratap_mls_2020}                                                      & \begin{tabular}[c]{@{}c@{}}\textbf{263,055} \\ 124,590 / 138,465 / --\end{tabular}                   & \begin{tabular}[c]{@{}c@{}}\textbf{1,096:43} \\ 520:13 / 576:29 / --\end{tabular}                  & \begin{tabular}[c]{@{}c@{}}\textbf{178} \\ 80 / 98 / --\end{tabular}                & \begin{tabular}[c]{@{}c@{}}\textbf{15\,s} \\ 15\,s / 15\,s / --\end{tabular}       &Read\\\bottomrule\\%\cdashline{1-6}

%&&&&& \\
\multicolumn{6}{c}{\textbf{Medium-clean dataset -- 2.7K}} \\ \hline
EPAC**$_{NC}$~\citep{old_esteve_epac_2010}                                                             & \begin{tabular}[c]{@{}c@{}}\textbf{623,250} \\ 465,859 / 157,391 / --\end{tabular}                  & \begin{tabular}[c]{@{}c@{}}\textbf{1,626:02} \\ 1,240:10 / 385:52 / --\end{tabular}                & \begin{tabular}[c]{@{}c@{}}\textbf{Unk} \\ -- / -- / --\end{tabular}           & \begin{tabular}[c]{@{}c@{}}\textbf{9\,s} \\ -- / -- / --\end{tabular}                       & \begin{tabular}[c]{@{}c@{}}Radio \\ Broadcasts\end{tabular}          \\\hline

\textbf{2.7k dataset total}                                                       & 
\begin{tabular}[c]{@{}c@{}}\textbf{886,305} \\ 590,449 / 295,856 / -\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{2,722:45} \\ 1,760:23 / 962:21 / -\end{tabular} & -                                                                       & -                                                                            & - \\\bottomrule\\
                                                    
\multicolumn{6}{c}{\textbf{Medium dataset -- 3K}} \\ \hline

\begin{tabular}[l]{@{}l@{}}African Accented \\ French$_{Apache 2.0}$~\citep{noauthor_african_2003}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{16,402} \\ 373 / 102 / 15,927\end{tabular}  & \begin{tabular}[c]{@{}c@{}}\textbf{18:56} \\ -- / -- / 18:56\end{tabular}                      & \begin{tabular}[c]{@{}c@{}}\textbf{232} \\ 48 / 36 / 148\end{tabular}         & %\begin{tabular}[c]{@{}c@{}}\textbf{4\,s} \\ -- / -- / --\end{tabular}                        &  Read\\
\begin{tabular}[c]{@{}c@{}}\textbf{4\,s} \\ -- / -- / --\end{tabular}                        &  Read\\\hline

Att-Hack$_{CC BY NC ND}$~\citep{le_moine_att-hack_2020}                                                           & \begin{tabular}[c]{@{}c@{}}\textbf{36,339} \\ 16,564 / 19,775 /  --\end{tabular}                     & \begin{tabular}[c]{@{}c@{}}\textbf{27:02} \\ 12:07 / 14:54 / --\end{tabular}                       & \begin{tabular}[c]{@{}c@{}}\textbf{20} \\ 9 / 11 / -- \end{tabular}                  & \begin{tabular}[c]{@{}c@{}}\textbf{2.7\,s}\\ 2.6\,s / 2.7\,s / --\end{tabular}                        & \begin{tabular}[c]{@{}c@{}}Acted \\ Emotional\end{tabular}          \\\hline

CaFE$_{CC NC}$~\citep{gournay_canadian_2018}                                                               & \begin{tabular}[c]{@{}c@{}}\textbf{936} \\ 468 / 468 / --\end{tabular}                              & \begin{tabular}[c]{@{}c@{}}\textbf{1:09} \\ 0:32 / 0:36 / --\end{tabular}                          & \begin{tabular}[c]{@{}c@{}}\textbf{12} \\ 6 / 6 / --\end{tabular}                   & \begin{tabular}[c]{@{}c@{}}\textbf{4.4\,s} \\ 4.2\,s / 4.7\,s / --\end{tabular}                        & \begin{tabular}[c]{@{}c@{}}Acted \\ Emotional\end{tabular}          \\\hline

%removed , \citep{cfpp2000_website}
\begin{tabular}[c]{@{}c@{}}CFPP2000$_{CC BY NC SA}$*\\ \citep{branca-rosoff_discours_2012}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{9853} \\ 166 / 1,184 / 8,503\end{tabular}                    & \begin{tabular}[c]{@{}c@{}}\textbf{16:26}\\ 0:14 / 1:56 / 14:16\end{tabular}                      & \begin{tabular}[c]{@{}c@{}}\textbf{49} \\ 2 / 4 / 43\end{tabular}                  & \begin{tabular}[c]{@{}c@{}}\textbf{6\,s}\\ 5\,s / 5\,s / 6\,s\end{tabular}                        & Spontaneous\\\hline

%removed , \citep{eslo_website}
ESLO2$_{NC}$~\citep{old_eshkol-taravella_grand_2011} & \begin{tabular}[c]{@{}c@{}}\textbf{62,918} \\ 30,440 / 32,147 / 331\end{tabular}                          & \begin{tabular}[c]{@{}c@{}}\textbf{34:12} \\ 17:06 / 16:57 / 0:09 \end{tabular}                          & \begin{tabular}[c]{@{}c@{}}\textbf{190} \\ 68 / 120 / 2\end{tabular}                & \begin{tabular}[c]{@{}c@{}}\textbf{1.9\,s} \\ 2\,s / 1.9\,s / 1.7\,s\end{tabular}                        & Spontaneous                                                          \\\hline
%EPAC**$_{NC}$~\citep{esteve_epac_2010}                                                             & \begin{tabular}[c]{@{}c@{}}\textbf{623,250} \\ 465,859 / 157,391 / --\end{tabular}                  & \begin{tabular}[c]{@{}c@{}}\textbf{1,626:02} \\ 1,240:10 / 385:52 / --\end{tabular}                & \begin{tabular}[c]{@{}c@{}}\textbf{1,935} \\ -- / -- / --\end{tabular}           & \begin{tabular}[c]{@{}c@{}}\textbf{9\,s} \\ -- / -- / --\end{tabular}                       & \begin{tabular}[c]{@{}c@{}}Radio \\

GEMEP$_{NC}$~\citep{old_banziger_introducing_2012}                                                              & \begin{tabular}[c]{@{}c@{}}\textbf{1,236} \\ 616 / 620 / --\end{tabular}                            & \begin{tabular}[c]{@{}c@{}}\textbf{0:50} \\ 0:24 / 0:26 / --\end{tabular}                          & \begin{tabular}[c]{@{}c@{}} \textbf{10} \\ 5 / 5 / --\end{tabular}                                                              & \begin{tabular}[c]{@{}c@{}}\textbf{2.5\,s} \\ 2.4\,s / 2.5\,s / --\end{tabular}                        & \begin{tabular}[c]{@{}c@{}}Acted \\ Emotional\end{tabular}          \\\hline

%old stats MPF
MPF~\citep{MPF_paper_2017}, \citep{MPF_ortolang}                                                                & \begin{tabular}[c]{@{}c@{}}\textbf{19,527} \\ 5,326 / 4,649 / 9,552\end{tabular}                          & \begin{tabular}[c]{@{}c@{}}\textbf{19:06} \\ 5:26 / 4:36 / 9:03\end{tabular}                            & \begin{tabular}[c]{@{}c@{}}\textbf{114}\\ 36 / 29 / 49\end{tabular}                 & \begin{tabular}[c]{@{}c@{}}\textbf{3.5\,s} \\ 3.7\,s / 3.6\,s / 3.4\,s\end{tabular}                        & Spontaneous                                                          \\\hline

\begin{tabular}[c]{@{}c@{}}PORTMEDIA$_{NC}$\\ (French)~\citep{old_lefevre_robustesse_2012}\end{tabular}    & \begin{tabular}[c]{@{}c@{}}\textbf{19,627} \\ 9,294 / 10,333 / --\end{tabular}                      & \begin{tabular}[c]{@{}c@{}}\textbf{38:59}\\ 19:08 / 19:50 / --\end{tabular}                        & \begin{tabular}[c]{@{}c@{}}\textbf{193} \\ 84 / 109 / --\end{tabular}               & \begin{tabular}[c]{@{}c@{}}\textbf{7.1\,s} \\ 7.4\,s / 6.9\,s / --\end{tabular}                        & \begin{tabular}[c]{@{}c@{}}Acted telephone \\ dialogue \end{tabular} \\\hline

%old stats TCOF
\begin{tabular}[c]{@{}c@{}}TCOF$_{CC BY NC SA}$\\(Adults)~\citep{TCOF_ortolang}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{58,722} \\ 10,377 / 14,763 / 33,582\end{tabular}                & \begin{tabular}[c]{@{}c@{}}\textbf{53:59} \\ 9:33 / 12:39 / 31:46\end{tabular}                     & \begin{tabular}[c]{@{}c@{}}\textbf{749} \\ 119 / 162 / 468\end{tabular}            & \begin{tabular}[c]{@{}c@{}}\textbf{3.3\,s} \\ 3.3\,s / 3.1\,s / 3.4\,s\end{tabular}                        & Spontaneous  \\\hline

\textbf{Medium dataset total}                                                       & 
\begin{tabular}[c]{@{}c@{}}\textbf{1,111,865} \\ 664,073 / 379,897 / 67,895\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{2,933:24} \\ 1,824:53 / 1,034:15 / 74:10\end{tabular} & -                                                                       & -                                                                            & -  
                                                    \\\bottomrule\\
                                                    %\cdashline{1-6}
%&&&&& \\
\multicolumn{6}{c}{\textbf{Large dataset -- 7K}} \\ \hline

%\begin{tabular}[c]{@{}c@{}}\textcolor{red}{CFPP2000}$_{CC BY NC SA}$*\\ \citep{branca-rosoff_discours_2012}, \citep{cfpp2000_website}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{12,574} \\ 203 / 1,686 / 10,685\end{tabular}                    & \begin{tabular}[c]{@{}c@{}}\textbf{20:20}\\ 0:16 / 2:35 / 17:28\end{tabular}                      & \begin{tabular}[c]{@{}c@{}}\textbf{50} \\ 2 / 4 / 44\end{tabular}                  & \begin{tabular}[c]{@{}c@{}}\textbf{5.8\,s}\\ 4.9\,s / 5.5\,s / 5.9\,s\end{tabular}                        & Spontaneous\\\hline

%\begin{tabular}[l]{@{}l@{}}\textcolor{red}{TCOF}$_{CC BY NC SA}$\\(Adults)~\citep{TCOF_ortolang}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{58,545} \\ 11,174 / 13,943 / 33,428 \end{tabular}                & \begin{tabular}[c]{@{}c@{}}\textbf{53:45} \\ 10:47 / 11:22 / 31:35\end{tabular}                     & \begin{tabular}[c]{@{}c@{}}\textbf{736} \\ 117 / 162 / 457 \end{tabular}            & \begin{tabular}[c]{@{}c@{}}\textbf{3\,s} \\ 3\,s / 2\,s / -- \end{tabular}                        & Spontaneous                                                          \\\hline

%\textcolor{red}{MPF}$_{NC}$~\citep{MPF_paper_2017}, \citep{MPF_ortolang}                                                                & \begin{tabular}[c]{@{}c@{}}\textbf{40,579} \\ 10,802 / 9,277 / 20,500\end{tabular}                          & \begin{tabular}[c]{@{}c@{}}\textbf{37:06} \\ 10:28 / 08:48 / 17:49\end{tabular}                            & \begin{tabular}[c]{@{}c@{}}\textbf{140}\\ 35 / 29 / 76\end{tabular}                 & \begin{tabular}[c]{@{}c@{}}\textbf{3\,s} \\ 3\,s / 3\,s / 3\,s\end{tabular}                        & Spontaneous  \\\hline

MaSS~\citep{boito-etal-2020-mass} & \begin{tabular}[c]{@{}c@{}}\textbf{8,219} \\ 8,219 / -- / -- \end{tabular}                            & \begin{tabular}[c]{@{}c@{}}\textbf{19:40} \\ 19:40 / -- / --\end{tabular} & \begin{tabular}[c]{@{}c@{}} \textbf{Unk} \\ -- / -- / --\end{tabular}                                                              & \begin{tabular}[c]{@{}c@{}}\textbf{8.6\,s} \\ 8.6\,s / -- / --\end{tabular}                        & Read        \\\hline

NCCFr$_{NC}$~\citep{torreira_nijmegen_2010} & \begin{tabular}[c]{@{}c@{}}\textbf{29,421} \\ 14,570 / 13,922 / 929 \end{tabular}                          & \begin{tabular}[c]{@{}c@{}}\textbf{26:35} \\ 12:44 / 12:59 / 00:50\end{tabular}                            & \begin{tabular}[c]{@{}c@{}}\textbf{46}\\ 24 / 21 / 1\end{tabular}                 & \begin{tabular}[c]{@{}c@{}}\textbf{3\,s} \\ 3\,s / 3\,s / 3\,s \end{tabular}                        & Spontaneous  \\\hline

\begin{tabular}[l]{@{}l@{}}Voxpopuli$_{CC0}$~\citep{wang2021voxpopuli}\\\textit{Unlabeled}\end{tabular}
    & \begin{tabular}[c]{@{}c@{}}\textbf{568,338} \\ -- / -- / --\end{tabular}                      & \begin{tabular}[c]{@{}c@{}}\textbf{4,532:17}\\ -- / -- / 4,532:17\end{tabular}                        & \begin{tabular}[c]{@{}c@{}}\textbf{Unk} \\ -- / -- / --\end{tabular}               & \begin{tabular}[c]{@{}c@{}}\textbf{29\,s} \\ -- / -- / --\end{tabular}                        & \begin{tabular}[c]{@{}c@{}}Professional speech \end{tabular} \\\hline
    
\begin{tabular}[l]{@{}l@{}}Voxpopuli$_{CC0}$~\citep{wang2021voxpopuli}\\\textit{transcribed}\end{tabular}
    & \begin{tabular}[c]{@{}c@{}}\textbf{76.281} \\ -- / -- / --\end{tabular}                      & \begin{tabular}[c]{@{}c@{}}\textbf{211:57}\\ -- / -- / 211:57\end{tabular}                        & \begin{tabular}[c]{@{}c@{}}\textbf{327} \\ -- / -- / --\end{tabular}               & \begin{tabular}[c]{@{}c@{}}\textbf{10\,s} \\ -- / -- / --\end{tabular}                        & \begin{tabular}[c]{@{}c@{}}Professional speech \end{tabular} \\\midrule

\textbf{Large dataset total***}                                                       & 
\begin{tabular}[c]{@{}c@{}}\textbf{1,814,242} \\ 682,322 / 388,217 / 99,084\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{7,739:22} \\ 1,853:02 / 1,041:07 / 4,845:07\end{tabular} & -                                                                       & -                                                                            & -  
                                                    
                                                    \\\bottomrule\\
                                                    %\cdashline{1-6}
%&&&&& \\
\multicolumn{6}{c}{\textbf{Extra Large dataset -- 14K}} \\ \hline
                                                    %\bottomrule

\begin{tabular}[l]{@{}l@{}}Audiocite.net$_{CC-BY}$~\citep{EVAINETAL_2022Audiocite}\end{tabular}
    & \begin{tabular}[c]{@{}c@{}}\textbf{817\,295} \\ 425\,033 / 159\,691 / 232\,571\end{tabular} 
    %& \begin{tabular}[c]{@{}c@{}}\textbf{6698:35}\\ 3477:24 / 1309:49 / 1911:21 \end{tabular}     
    & \begin{tabular}[c]{@{}c@{}}\textbf{6698:35}\\ 3477:24 / 1309:49 / 1911:21 \end{tabular}
    & \begin{tabular}[c]{@{}c@{}}\textbf{130} \\ 35 / 32 / 63\end{tabular}  
%   & \begin{tabular}[c]{@{}c@{}}\textbf{466} \\ 150 / 141 / 175\end{tabular}            
    & \begin{tabular}[c]{@{}c@{}}\textbf{29\,s} \\ 29\,s / 29\,s / 29\,s\end{tabular}                      
    & \begin{tabular}[c]{@{}c@{}} Read \end{tabular} \\\midrule

\begin{tabular}[l]{@{}l@{}}Niger-Mali Audio Collection $_{CC BY NC ND}$~\citep{ZANONBOITOETAL_2022NigerMaliAudio} \citep{ZANONBOITOETAL_2022SpeechResourcesTamasheq} \end{tabular}
    & \begin{tabular}[c]{@{}c@{}}\textbf{38\,332} \\ 18\,546 / 19\,786 / --\end{tabular}                    
    & \begin{tabular}[c]{@{}c@{}}\textbf{111:01}\\ 52:15 / 58:46 / --\end{tabular}                        
    & \begin{tabular}[c]{@{}c@{}}\textbf{357} \\ 192 / 165 / --\end{tabular}               
    & \begin{tabular}[c]{@{}c@{}}\textbf{10\,s} \\ 10\,s / 10\,s / --\end{tabular}                      & \begin{tabular}[c]{@{}c@{}} Radio broadcasts \end{tabular} \\\midrule
    
\textbf{Extra Large dataset total}                                                       & 
\begin{tabular}[c]{@{}c@{}}\textbf{2\,669\,869} \\ 1\,125\,901 / 567\,694 / 331\,655 \end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{14\,548:58} \\ 5\,382:41 / 2\,409:42 / 6\,756:28 \end{tabular} & -                                                                       & -                                                                            & -  
                                                    \\\bottomrule                                                    
\end{tabular}}
 \\\raggedright \scriptsize{*Composed of audio files not included in the CEFC corpus v2.1, 02/2021; **speakers are not uniquely identified.; ***Stats of CFPP2000, MPF and TCOF have changed a bit due to a change in data extraction; License: CC=Creative Commons; NC=non-commercial; BY= Attribution; SA= Share Alike; ND = No Derivative works; CC0 = No Rights Reserved}  
    \label{tab:medium_and_small_datasets}
\end{table*}




==> tables/energy.tex <==
\begin{table}[!th]
\caption{Estimates of the energy in kilowatt hour (kwH) and CO$_2$ equivalent in kilogram produced by the training of the \nameprojectnew models.}
\begin{center}
    \begin{tabular}{lcccc}
        % \hline
        \toprule
        % \multicolumn{5}{|c|}{\textbf{Full End-to-End models (1 step)}} \\
        % \hline
        \textbf{Model} & \textbf{Train. Time} & \textbf{GPUs} & \textbf{Energy} & \textbf{CO$_2$} \\  & \textit{(hours)} &  & \textit{(kWh)} & \textit{(kg)} \\
        \hline
        
        1K-\textit{base} & 250 & 4 Tesla V100 & 195.0 & 10.5 \\
        1K-\textit{large} & 925 & 4 Tesla V100 & 721.5 & 37.5   \\
        2.7K-\textit{base} & 128 & 32 Tesla V100 & 682.2 & 35.4  \\
        3K-\textit{base} & 128  & 32 Tesla V100 & 682.2 & 35.4  \\
        3K-\textit{large} & 341  & 32 Tesla V100 & 1,817.5 & 94.5  \\
        7K-\textit{base} & 123  & 64 Tesla V100 & 1,535.0 & 79.8 \\
        7K-\textit{large} & 211  & 64 Tesla V100 & 4,501.0 & 234 \\
        14K-\textit{light} & 156  & 32 Tesla V100 & 1,497.6 & 77.8  \\
        14K-\textit{large} & 436 & 64 Tesla V100 & 8,371.2 & 435  \\
        14K-\textit{xlarge} & 525 & 104 Tesla A100 & 16,511.2 & 859  \\
        \bottomrule\\
    \end{tabular}
\end{center}
\label{tab:energy}
\end{table}

==> tables/genderstudy_mtedx.tex <==
\begin{table}
\centering
%\resizebox{\columnwidth}{!}{
\scalebox{0.80}{
\begin{tabular}{l|lccc|c}\toprule
\multicolumn{6}{c}{\textbf{Balanced Dataset (ASR) }}                              \\
%\multicolumn{6}{c}{\textbf{Original Content (fr-fr)}}                              \\
                       & \multicolumn{1}{c}{} & \textbf{M}         & \textbf{F}        & \textbf{B}    & \textbf{All}       \\\midrule
%\multirow{2}{*}{train} & \# speakers          & 550       & 388      & 4       & 942       \\
 %                      & Duration             & 100:02 & 68:28 & 0:44 & 169:14 \\
%\multirow{2}{*}{valid} & \# speakers          & 5         & 7        & -       & 12        \\
 %                      & Duration             & 0:38   & 1:00  & -       & 1:38   \\
%\multirow{2}{*}{test}  & \# speakers          & 6         & 4        & -       & 10        \\
 %                      & Duration             & 0:54   & 0:39  & -       & 1:33   %\\\midrule
%                       & \multicolumn{1}{c}{} & \textbf{M}         & \textbf{F}        & \textbf{B}    & \textbf{ALL}       \\

\multirow{2}{*}{train} & \# speakers          & 332       & 342      & -       & 674       \\
                       & Duration             & 30:15  & 30:15 & -       & 60:30  \\
\multirow{2}{*}{valid} & \# speakers          & 7        & 7        & -       & 16        \\
                       & Duration             & 0:30   & 0:30  & -       & 1:00  \\
\multirow{2}{*}{test} & \# speakers          & 50        & 50        & -       & 100        \\
                       & Duration             & 8:53   & 8:36  & -       & 17:29  \\\midrule
\multicolumn{6}{c}{\textbf{Translation Dataset (ST) }}                              \\
%                                        &             & \textbf{M} & \textbf{F} & \textbf{B} & \textbf{ALL} \\
\midrule
\multirow{2}{*}{train} & \# speakers & 146        & 102        & 2             & 250          \\
                                        & Duration    & 26:28   & 18:14   & 0:22       & 45:04     \\
\multirow{2}{*}{valid} & \# speakers          & 5         & 7        & -       & 12        \\
                       & Duration             & 0:38   & 1:00  & -       & 1:38   \\
\multirow{2}{*}{test}  & \# speakers          & 6         & 4        & -       & 10        \\
                       & Duration             & 0:54   & 0:39  & -       & 1:33   \\\midrule
\end{tabular}}
\caption{Statistics for the datasets used for the tasks~(M=male;F=female;B=speakers of both genders present). Duration written as hours:minutes. \textbf{MISSING ASV}}
\label{gs:tab:asrdata}
\end{table}
